Blending Is All You Need: Cheaper, Better Alternative to Trillion-Parameters LLM

In conversational AI research, there's a noticeable trend towards developing models with a larger number of parameters, exemplified by models like ChatGPT. While these expansive models tend to generate increasingly better chat responses, they demand significant computational resources and memory. This study explores a pertinent question: Can a combination of smaller models collaboratively achieve comparable or enhanced performance relative to a singular large model? We introduce an approach termed "blending", a straightforward yet effective method of integrating multiple chat AIs. Our empirical evidence suggests that when specific smaller models are synergistically blended, they can potentially outperform or match the capabilities of much larger counterparts. For instance, integrating just three models of moderate size (6B/13B paramaeters) can rival or even surpass the performance metrics of a substantially larger model like ChatGPT (175B+ paramaters). This hypothesis is rigorously tested using A/B testing methodologies with a large user base on the Chai research platform over a span of thirty days. The findings underscore the potential of the "blending" strategy as a viable approach for enhancing chat AI efficacy without a corresponding surge in computational demands.

==> old_related_work.tex <==
\section{Related Work}

\subsection{Chat AI approaches}

ChatAIs have been developed for a variety of applications, from user assistance to casual interactions (for \textit{chitchat})~\cite{10.1145/3166054.3166058}. Early designs were based on rule-based algorithms~\cite{10.1145/365153.365168}. As research progressed, there was a movement towards retrieval-based models, which later integrated with generative techniques~\cite{nlp4convai-2021-natural}. The emergence of pre-trained language models, especially those built on Transformer architectures, marked a significant change in chat AI development~\cite{zhu2022simple, NIPS2017_3f5ee243, 10.1145/3373017.3373028}. Due to the large performance gains, recent trends show a general reliance on increasingly larger Transformer-based models finetuned on extensive conversational datasets for the development and deployment of chat AIs~\cite{ DBLP:journals/corr/abs-2001-09977, roller-etal-2021-recipes, DBLP:journals/corr/abs-2006-16779, choudhary-kawahara-2022-grounding, yan2022deep}.

Traditional training techniques primarily used conversational datasets as an unsupervised source of data. However, newer methodologies highlight the importance of human feedback in training to align better with human expectations of an engaging conversation~\cite{DBLP:journals/corr/abs-1811-07871, DBLP:journals/corr/abs-2112-00861, DBLP:journals/corr/abs-2001-09768}. The methodology used by InstructGPT~\cite{ouyang2022training}, which employs reinforcement learning from human feedback \citep[RLHF;][]{christiano2017deep, stiennon2020learning}, exemplifies this shift. Within this framework, a reward model is trained using user-ranked responses. This model then facilitates reinforcement learning, where the chat AI acts as an agent within its environment. An alternative method avoids adjustments to model parameters during reinforcement by using proximal policy optimization. Instead, the reward model is used during inference to filter out undesired responses~\citep{DBLP:journals/corr/abs-1912-02164}. Additionally, methods including constrained optimization, control codes, and expert iteration have been explored, incorporating human feedback into the chat AI training process~\cite{DBLP:journals/corr/AchiamHTA17, DBLP:journals/corr/abs-1909-05858, DBLP:journals/corr/abs-1712-01815, DBLP:journals/corr/AnthonyTB17}.

Finally, \citet{irvine2023rewarding} demonstrated that explicit incorporation of reward models trained on a variety of human feedback mechanisms can be used to develop a highly engaging Chat AI, resulting in high levels of user retention - the main objective of commercially deployed Chat AIs. We further demonstrate that an improved ChaiAI model proposed in this work is able to out-perform all existing state of the art chat AIs by \textit{blending} the output responses from many smaller chat AI systems to create a richer and more engaging overall conversation. 


\subsection{Combining Generative systems}

In this work, ChaiAI demonstrates that by \textit{blending} many smaller chat AI systems, the overall system performs better than any other state-of-the-art large singular system. This section discusses the range of approaches proposed in literature to combine/ensemble a set of systems for generative sequence-to-sequence tasks, such as in the conversational setting. 

Combination of multiple models has become a standard approach to improve the performance of deep learning systems. Typically a set of individual system can be constructed from a single base learner using methods such as bagging \cite{breiman1996bagging}, boosting \cite{liu2014facial, zhang2020snapshot}, and inference-time dropout \cite{srivastava2014dropout, gal2016dropout}. However it is shown that a heterogeneous set of more diverse individual models constructed using different base learners can allow for a better performing combined system \cite{kilimci2018deep, seijo2017ensemble}. To combine the individual systems, a variety of methods, such as stacking \cite{wolpert1992stacked} and negative correlation learning \cite{liu1999ensemble} have been proposed in literature. Nevertheless, in classification tasks, the individual systems are usually combined by max-voter schemes \cite{ju2018relative, simonyan2014very} or a simple unweighted average over the different classifier outputs \cite{he2016deep, bann2022l2, raina_gales_knill_2020, szegedy2015going}. However, for natural language generative systems, where sequential and discrete-space outputs such as conversational responses consist of a sequence of tokens, such simple combinations of ensembles are inapplicable and meaningless.



Despite the challenge of sequence-level combination, for the task of grammatical error correction, \citet{tarnavskyi-etal-2022-ensembling} exploit the specific nature of the task to benefit from a \textit{max voting} scheme, where only edits predicted by the majority of individual systems are retained to construct a single combined output sequence. As a more generic approach, token-level ensembles (often termed product of expectations), \cite{sennrich2015improving, freitag2017ensemble, malinin2021uncertainty, gec-ensemble-dist} can be used to combine decoder outputs by averaging the probabilities over the token predictions during decoding.

However, the above mentioned approaches often assume identical architectures (homogenous base learners) for the different systems as well as white-box access to the internals of a system. With an increasing trend of limited blackbox access to large language models (e.g. ChatGPT~\cite{liu2023summary} and BARD \cite{Nyberg_2021}), it is meaningful to consider system combination approaches where there is only access to the output sequences. As a response to this challenge, in the domain of automatic speech recognition, \citet{consensus-decoding} select a single output using a simple Minimum Bayes' Risk (MBR) decoding approach~\citep{kumar-byrne-2004-minimum}. This approach has also shown some success in recent machine translation approaches~\citep{rosti-etal-2007-combining, rosti-etal-2007-improved, freitag-etal-2022-high} and summarisation \cite{manakul2023cued}. In this work we further demonstrate that systems can be effectively combined to significantly increase user engagement for conversational interactions by stochastically selecting responses from different systems at every turn of the conversation. These observations are well aligned with the traditional motivations for ensembling: a combined system is able to benefit from the individual strengths of each component system.

